Adaptation Needs in Robotic Systems: Assessing Behavior Trees and Their Enhancement

Robotic systems increasingly operate in dynamic, uncertain, and open-ended environments, where design-time assumptions may no longer hold, and adaptation becomes necessary to maintain effective and safe operation. Behavior Trees (BTs) are widely used in robotic control architectures due to their modularity, readability, and reactivity. This raises a central question: are BTs sufficient to meet the adaptation needs of modern robotic systems? This paper investigates this question through a literature-driven study complemented by empirical validation. First, we derive a classification of robotic adaptation needs from the literature, organizing them into six categories: Knowledge, Perception, Actuation, System, Mission, and Environment. Then, we analyze the capabilities and limitations of classical BTs with respect to these needs. Then, we characterize BT-based approaches for adaptation from the existing literature and organize them into four primary families, i.e., generation, extension, evolution, and refinement, including approaches that combine multiple families. Our analysis shows that the modularity, flexibility, and reactivity of classical BTs are insufficient for adaptation needs involving runtime restructuring, reasoning under uncertainty, mission reinterpretation, learning, or integration with external knowledge and planning mechanisms. Enhanced BT approaches address several of these limitations, but to different extents and often with limitations of their own. Our findings relate adaptation needs to both the capabilities and limitations of classical and enhanced BTs, providing guidance on when classical BTs are sufficient, when enhanced mechanisms are needed, and which challenges remain or emerge for adaptive robotic control architectures.

==> sections/Tables4Validation.tex <==
Tb\ref{tbl:bt_reasons}
\ref{tbl:uncertainty-sources}

\begin{table}[t]
\centering
\caption{Limitations on adaptability and extensibility of BTs}
\label{tbl:bt_reasons}
\small
\begin{tabular}{p{1.3cm}|p{6.5cm}}
\hline
\textbf{Limitation} & \textbf{Description} \\
\hline
L1 & Static control flow in Classic BTs limits runtime flexibility~\cite{pezzato2023active, rovida2017extended}. \\
\hline
L2 & Fixed execution order prevents flexible adaptation to runtime changes~\cite{rovida2017extended, fusaro2021human}. \\
\hline
L3 & Traditional BTs operate under deterministic assumptions, which are unsuitable for uncertain environments~\cite{fusaro2021human, rostamnia2025towards,abiyev2016robot,behery2023human}. \\
\hline
L4 & Difficulty handling partial observability and incomplete state information~\cite{li2022towards, pezzato2023active}. \\
\hline
L5 & Human-centered and collaborative industrial environments introduce uncertainty and variability not captured by Classic BTs~\cite{behery2023human, fusaro2021human}. \\
\hline
L6 & Suboptimal execution and lack of explicit representation of the purpose and intent of behaviors~\cite{rovida2017extended}. \\
\hline
L7 & Modeling conditions as explicit nodes are unsuitable for planning-based domains~\cite{rovida2017extended}. \\
\hline
L8 & Challenges in representing and managing highly complex behaviors~\cite{pezzato2023active}. \\
\hline
L9 & Limited explainability, particularly in diagnosing and explaining execution failures~\cite{lemasurier2024reactive}. \\
\hline
L10 & Lack of mechanisms for task resumption after interruptions or failures~\cite{el2021resume}. \\
\hline
L11 & Architectural adaptation of BTs often focuses on functional goals while neglecting quality requirements~\cite{alberts2024rebet,wang2020extending}. \\
\hline
L12 & Difficulty in handling continuous-valued states and actions~\cite{abiyev2016robot}. \\
\hline
\end{tabular}
\end{table}




\begin{table*}[h!]
\centering
\caption{Mapping adaptation needs to approaches.}
\label{tbl:uncertainty-sources}
\begin{tabular}{p{1.4cm}|p{3.3cm}|p{1.2cm}|p{3.6cm}|p{2.4cm}|p{1.6cm}|p{1.5cm}}
\hline
\textbf{Category} & \textbf{Subtype} & Evolution & Extension & Generation & Refinement &  \\
\hline
\multirow{3}{*}{Knowledge} 
 & Abstraction &  &  & & & \\
 \cline{2-7}
 & Incompleteness & \cite{hallawa2017instinct} & \cite{li2022towards} &\cite{iovino2023framework} & & \cite{scherf2023interactively}\\
 \cline{2-7}
 & Inaccuracy&  & &  & & \cite{scherf2023interactively}\\
 \cline{2-7}
 & Driftness& \cite{scheper2016behavior} & & \cite{ruiz2022automating}& &\\
 \cline{2-7}
\hline
\multirow{3}{*}{Perception}
 & Multipicity & &  &  & &  \\
 \cline{2-7}
 & Inaccuracy & &  &  & &  \\
 \cline{2-7}
 & Unavailability &  &  & & & \\
  \hline
\multirow{2}{*}{Actuation}
 & Non-determinism & &  &  & & \cite{scherf2023interactively} \\
 \cline{2-7}
 & Unavailability &  &  & & & \\
  \hline
\multirow{4}{*}{System}
 & Component failure &  & \cite{el2021resume,wang2020extending} & \cite{segura2017integration} & &  \\
 \cline{2-7}
 & Changing resources & \cite{chen2023co} &\cite{alberts2024rebet} & & &  \\
 \cline{2-7}
 & New resources & &  &  & &  \\
 \cline{2-7}
 & Communication impairement & &  &  & &  \\
  \hline 
\multirow{5}{*}{Mission}
 & Uncertaint specification & \cite{montague2024hierarchical,hallawa2020evolving}&\cite{fusaro2021human,rovida2017extended,behery2023human,rostamnia2025towards} &\cite{iovino2023framework,colledanchise2018learning,deng2023learning} & \cite{deng2023learning}&-\\
 \cline{2-7}
& Future mission changes & &  &  & &  \\
 \cline{2-7}
 & Outdated mission & &  &  & &  \\
 \cline{2-7}
 & Uncertain quality goals &  &  & & & \\
 \cline{2-7}
 & Uncertain relationships &  &  & & & \\
\hline
\multirow{3}{*}{Environment}
 & Execution context changes& \cite{hallawa2017instinct} & \cite{pezzato2023active,fusaro2021human,li2022towards,alberts2024rebet,wang2020extending,rostamnia2025towards} & \cite{wen2024auction,iovino2023framework,verma2021automatic,zhou2024llm,herranz2022decentralised,segura2017integration} & &\cite{scherf2023interactively}\\
 \cline{2-7}
 & Non-humans agent coexistence & & \cite{abiyev2016robot} &  & &  \\
 \cline{2-7}
 &Human agents coexistence & &  \cite{pezzato2023active,fusaro2021human,el2021resume,behery2023human,li2022towards}&\cite{ruiz2022automating,chen2024integrating} & \cite{verdaguer2025boosting}& \\
\hline
\end{tabular}
\end{table*}


==> sections/validation.tex <==
%\section{Validation}\label{sec:validation}



